Highly reflective white clouds on the western dayside of an exo-Neptune

Highly-irradiated gas giant exoplanets are predicted to show circulation patterns dominated by day-to-night heat transport and a spatial distribution of clouds that is driven by advection and local heating. Hot-Jupiters have been extensively studied from broadband phase-curve observations at infrared and optical wavelengths, but spectroscopic observations in the reflected light are rare and the regime of smaller and higher-metallicity ultra-hot planets, such as hot-Neptunes, remains largely unexplored to date. Here we present the phase-resolved reflected-light and thermal-emission spectroscopy of the ultra-hot Neptune LTT 9779b, obtained through observing its full phase-curve from 0.6 to 2.8 $\mu$m with JWST NIRISS/SOSS. We detect an asymmetric dayside in reflected light (3.1$\sigma$ significance) with highly-reflective white clouds on the western dayside (A = 0.79$\pm$0.15) and a much lower-albedo eastern dayside (A = 0.41$\pm$0.10), resulting in an overall dayside albedo of A = 0.50$\pm$0.07. The thermal phase curve is symmetric about the substellar point, with a dayside effective temperature of T$_\mathrm{eff,day}$ = 2,260$^{+40}_{-50}$ K and a cold nightside (T$_\mathrm{eff,night}$ <1,330 K at 3-$\sigma$ confidence), indicative of short radiative timescales. We propose an atmospheric circulation and cloud distribution regime in which heat is transported eastward from the dayside towards the cold nightside by an equatorial jet, leading to a colder western dayside where temperatures are sufficiently low for the condensation of silicate clouds.

==> commanddef.tex <==
\newcommand\ion[2]{#1$\,${\scshape{#2}}}  % ion, i.e., CII = \ion{C}{ii}
\newcommand{\vect}[1]{\mathbf{#1}}
\newcommand{\mt}[1]{\mathrm{#1}}
\newcommand{\Msun}{\ensuremath{\,M_{\odot}}}
\newcommand{\Mearth}{\ensuremath{\,M_{\oplus}}}
\newcommand{\Mmoon}{\ensuremath{\,M_{\mathrm{Moon}}}}
\newcommand{\Mjup}{\ensuremath{\,M_{\mathrm{Jup}}}}
\newcommand{\Rjup}{\ensuremath{\,R_{\mathrm{Jup}}}}
\newcommand{\mum}{\ensuremath{\,\mu}m}
\newcommand{\arcmin}{\ensuremath{^{\prime}}}
\newcommand{\arcsec}{\ensuremath{^{\prime\prime}}}
\newcommand{\farcmin}{\mbox{\ensuremath{.\mkern-4mu^\prime}}}%  % fractional arcminute symbol: 0.'0
\newcommand{\farcsec}{\mbox{\ensuremath{\,.\!\!^{\prime\prime}}}}%  % fractional arcsecond symbol: 0.''0
\newcommand{\water}{H$_{2}$O}

